By Land, Air, or Sea: Multi-Domain Robot Communication Via Motion

In this paper, we explore the use of motion for robot-to-human communication on three robotic platforms: the 5 degrees-of-freedom (DOF) Aqua autonomous underwater vehicle (AUV), a 3-DOF camera gimbal mounted on a Matrice 100 drone, and a 3-DOF Turtlebot2 terrestrial robot. While we previously explored the use of body language-like motion (called kinemes) versus other methods of communication for the Aqua AUV, we now extend those concepts to robots in two new and different domains. We evaluate all three platforms using a small interaction study where participants use gestures to communicate with the robot, receive information from the robot via kinemes, and then take actions based on the information. To compare the three domains we consider the accuracy of these interactions, the time it takes to complete them, and how confident users feel in the success of their interactions. The kineme systems perform with reasonable accuracy for all robots and experience gained in this study is used to form a set of prescriptions for further development of kineme systems.

==> figures/confusion_overall.tex <==
\newcommand\items{11}   %Number of classes
\arrayrulecolor{white} %Table line colors

\begin{table*}[]
    \centering
\noindent\begin{tabular}{cr*{\items}{|E}|}
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{\items}{c}{\textbf{Kinemes Identified}} \\ \hhline{~*\items{|-}|}
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{\rot{Affirmative}} & 
\multicolumn{1}{c}{\rot{Negative}} & 
\multicolumn{1}{c}{\rot{Follow Me}} & 
\multicolumn{1}{c}{\rot{Indicate Motion (Left)}} & 
\multicolumn{1}{c}{\rot{Indicate Motion (Right)}} & 
\multicolumn{1}{c}{\rot{Indicate Object (Left)}} & 
\multicolumn{1}{c}{\rot{Indicate Object (Right)}} & 
\multicolumn{1}{c}{\rot{Indicate Stay}} & 
\multicolumn{1}{c}{\rot{Danger}} & 
\multicolumn{1}{c}{\rot{Malfunction}} & 
\multicolumn{1}{c}{\rot{Repeat Last}} \\ \hhline{~*\items{|-}|}
\multirow{\items}{*}{\rotatebox{90}{\textbf{Kinemes Shown}}} 
&Affirmative                        & 19 & 0  & 0  & 0  & 0  & 0  & 0  & 0  & 0  & 1  & 0 \\ \hhline{~*\items{|-}|}
&Negative                         & 3  & 16 & 0  & 0  & 0  & 0  & 0  & 0  & 0  & 0  & 0\\ \hhline{~*\items{|-}|}
&Follow Me                  & 3  & 0  & 17 & 3  & 2  & 4  & 1  & 1  & 0  & 0  & 0\\ \hhline{~*\items{|-}|}
&Indicate Motion (Left)     & 0  & 0  & 1  & 23 & 0  & 0  & 0  & 1  & 0  & 0  & 1\\ \hhline{~*\items{|-}|}
&Indicate Motion (Right)    & 0  & 0  & 3  & 0  & 19 & 0  & 0  & 0  & 0  & 0  & 0\\ \hhline{~*\items{|-}|}
&Indicate Object (Left)     & 4  & 0  & 0  & 0  & 0  & 11 & 0  & 3  & 0  & 0  & 0\\ \hhline{~*\items{|-}|}
&Indicate Object (Right)    & 4  & 0  & 1  & 0  & 1  & 0  & 10 & 2  & 1  & 0  & 0\\ \hhline{~*\items{|-}|}
&Indicate Stay              & 0  & 0  & 1  & 0  & 1  & 0  & 0  & 21 & 0  & 0  & 0\\ \hhline{~*\items{|-}|}
&Danger                     & 0  & 1  & 0  & 0  & 0  & 0  & 0  & 4  & 17 & 4  & 1\\ \hhline{~*\items{|-}|}
&Malfunction                & 1  & 0  & 0  & 0  & 0  & 0  & 0  & 0  & 2  & 17 & 1\\ \hhline{~*\items{|-}|}
&Repeat Last                & 0  & 0  & 3  & 3  & 0  & 3  & 3  & 3  & 0  & 2  & 6\\ \hhline{~*\items{|-}|}
\end{tabular}
\hspace{30mm}
    \caption{Confusion matrix for kineme identification across all systems.}
    \label{tab:confusion_overall}
\end{table*}



==> src/notused.tex <==
\subsection{Domain Differences}
We explore the use of kinemes in the domains of underwater, aerial, and terrestrial robotics. 
The original motivation for the use of kinemes underwater was the lack of good communication vectors underwater: audio is distorted, digital displays are hard to read, and lights are difficult to understand and disorienting, and no radio or wireless signals work at any reasonable distance.. 
This motivation is less relevant to the aerial and terrestrial robots, as there are some feasible communication vectors in those domains.
Digital displays and text-to-speech (TTS) systems would be reasonable in both cases, and wireless or radio connectivity is also possible.
This does not, however mean that kineme communication is pointless in these domains: far from it.
In the case of aerial robots, kinemes would enable communication at further distances than digital displays, have no issue with being drowned out by propeller noise as TTS systems would, and provide an alternative to radio communications. 
Additionally, in the case of both aerial and terrestrial robots, while kinemes may not outperform the traditional communication vectors in this domain, kinemes provide an interesting alternative to them.
Kineme communication transcends written and spoken language and taps in to a capability that most humans share: reading body language implicitly.  
Either as the primary or a side channel of communication, kinemes are still worth exploring in these other domains which have other feasible communication vectors.

\input{figures/kineme_list.tex}

\subsection{Areas of Exploration}
The focus of this work is the exploration of the effectiveness of kinemes in physically-grounded interactions with users in the three chosen domains. 
We want to explore how accuracy, average time to complete interaction, and confidence in interaction correctness vary based on kineme and the system involved, comparing across domain and kineme.
In this work, we do not compare kineme communication to traditional communication vectors in each field.
This is a larger questions which we intend to address in future work, but is not addressed here.
Therefore, our central question is this: \enquote*{How well do different kinemes perform on different robots and in different domains?}
